Vortex Nucleation in a Bose-Einstein Condensate: From the Inside Out

We observed a new mechanism for vortex nucleation in Bose-Einstein condensates (BECs) subject to synthetic magnetic fields. We made use of a strong synthetic magnetic field initially localized between a pair of merging BECs to rapidly create vortices in the bulk of the merged condensate. Unlike previous implementations and in agreement with our Gross-Pitaevskii equation simulations, our dynamical process rapidly injects vortices into our system's bulk, and with initial number in excess of the system's equilibrium vortex number.

==> Draft Arxiv/macros.tex <==

%%
%% macros
%%

% Length

\def\nm{{\ {\rm nm}}}                       % nm
\def\mm{{\ {\rm mm}}}                       % mm
\def\cm{{\ {\rm cm}}}                       % cm
\def\micron{{\ \mu{\rm m}}}                 % Microns
\def\um{{\ \mu{\rm m}}}                 % Microns
\def\angstrom{{\ \mbox{{\rm \AA}}}}         % Angstroms

% Electrons
\def\tesla{{\ {\rm T}}}                     % tesla
\def\nohm{{\ {\rm n}\Omega}}                % nohm
\def\uohm{{\ \mu\Omega}}                    % uohm
\def\mohm{{\ {\rm m}\Omega}}                % mohm
\def\ohm{{\ \Omega}}                        % ohm
\def\kohm{{\ {\rm k}\Omega}}                % Kohm
\def\Mohm{{\ {\rm M}\Omega}}                % Mohm
\def\conductance#1{{\times{#1}\ \Omega^{-1}}} % Mhos

\def\density#1{{\times{#1}\ {\rm cm}^{-2}}}             % Density
\def\mobility#1{{\times{#1}\ {\rm cm}^{2}/{\rm V s}}}   % Mobility
\def\microvolt{{\ \mu{\rm V}}}              % Microvolts
\def\volt{{\ {\rm V}}}                      % volts

% Energy
\def\eV{{\ {\rm eV}}}                       % eV
\def\meV{{\ {\rm meV}}}                     % meV
\def\ueV{{\ \mu{\rm eV}}}                   % ueV
\def\neV{{\ {\rm neV}}}                     % neV

% Frequency
\def\uHz{{\ \mu{\rm Hz}}}                   % uHz
\def\mHz{{\ {\rm mHz}}}                     % mHz
\def\Hz{{\ {\rm Hz}}}                       % Hz
\def\kHz{{\ {\rm kHz}}}                     % kHz
\def\MHz{{\ {\rm MHz}}}                     % MHz
\def\GHz{{\ {\rm GHz}}}                     % GHz
\def\THz{{\ {\rm THz}}}                     % THz

% Time
\def\fs{{\ {\rm fs}}}                       % fs
\def\ps{{\ {\rm ps}}}                       % ps
\def\ns{{\ {\rm ns}}}                       % ns
\def\us{{\ \mu{\rm s}}}                     % us
\def\ms{{\ {\rm ms}}}                       % ms
\def\second{{\ {\rm s}}}                    % s

% Temperature
\def\kelvin{{\ {\rm K}}}                    % K
\def\mK{{\ {\rm mK}}}                       % mK
\def\uK{{\ \mu{\rm K}}}                     % uK
\def\nK{{\ {\rm nK}}}                       % nK

% Magnetic Field
\def\tesla{{\ {\rm T}}}                 % T
\def\mT{{\ {\rm mT}}}                       % mT
\def\uT{{\ \mu{\rm T}}}                     % uT
\def\nT{{\ {\rm nT}}}                       % nT

% AMO abbriviations
\def\Er{{{E_L}}}                            % Er
\def\kr{{{k_L}}}                            % kr
\def\Rb87{^{87}\rm{Rb}}                 % Rb 87
\def\Li6{^{6}\rm{Li}}                   % Rb 87
\def\UoverTC{(U/t)_{\rm c}}                 % t/U_c

\def\nbar{\left<{\hat n}_k\right>}                  % average number
\def\nbarexpt{\left<n(k_x,k_y)\right>}              % average number

% Specific Symbols
\def\DeltaSAS{{\Delta_{{\rm SAS}}}}         % DeltaSAS
\def\HeFour{{^4{\rm He}}}                   % Helium 4
\def\HeThree{{^3{\rm He}}}                  % Helium 3
\def\lb{{l_B}}                              % Magnetic Length
\def\DoverL{{d/\lb}}                        % d/l
\def\DoverLcrit{{\DoverL_{\rm crit}}}       % d/l_crit
\def\Bpar{{B_{\|}}}                         % B Parallel
\def\Bperp{{B_{\perp}}}                     % B Perpindicular
\def\AlGaAs#1#2{{{\rm Al}_{#1}{\rm Ga}_{#2}{\rm As}}} % Al_xGa_{1-x}As
\def\Schrodinger{{Schr\"odinger\ }}

\def\squigma{\xi}

% Basic mathematical symbols
\def\ex{{\mathbf e}_x}                            % e_x
\def\ey{{\mathbf e}_y}                            % e_y
\def\ez{{\mathbf e}_z}                            % e_z
\def\er{{\mathbf e}_r}                            % e_r
\def\epos{{\mathbf e}_+}                            % e_z
\def\eneg{{\mathbf e}_-}                            % e_z
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\def\ud{{\uparrow\downarrow}}
\def\du{{\downarrow\uparrow}}
\def\udc{{\uparrow,\downarrow}}
\def\duc{{\downarrow,\uparrow}}

% Some compressed symbols
\def\shorttimes{\!\times\!}                          
\def\shorteq{\!=\!}                          
\def\shortapprox{\!\approx\!}                          
\def\shortminus{\!-\!}                           


% Commands for bra-ket notation
\newcommand{\bra}[1]{\left< #1\right|}
\newcommand{\ket}[1]{\left|#1\right>}
\newcommand{\braket}[2]{\langle #1|#2\rangle}
\newcommand{\braP}[1]{\langle\langle#1|}
\newcommand{\ketP}[1]{|#1\rangle\rangle}
\newcommand{\braketP}[2]{\langle\langle#1|#2\rangle\rangle}

% Compact around figures
\addtolength{\abovecaptionskip}{-0.15in}
\addtolength{\belowcaptionskip}{-0.15in}

%%
%% End of my macros
%%
